How Effective are Large Language Models in Generating Software Specifications?

Software specifications are essential for many Software Engineering (SE) tasks such as bug detection and test generation. Many existing approaches are proposed to extract the specifications defined in natural language form (e.g., comments) into formal machine readable form (e.g., first order logic). However, existing approaches suffer from limited generalizability and require manual efforts. The recent emergence of Large Language Models (LLMs), which have been successfully applied to numerous SE tasks, offers a promising avenue for automating this process. In this paper, we conduct the first empirical study to evaluate the capabilities of LLMs for generating software specifications from software comments or documentation. We evaluate LLMs performance with Few Shot Learning (FSL) and compare the performance of 13 state of the art LLMs with traditional approaches on three public datasets. In addition, we conduct a comparative diagnosis of the failure cases from both LLMs and traditional methods, identifying their unique strengths and weaknesses. Our study offers valuable insights for future research to improve specification generation.

==> images/baseline_rootcause.tex <==


\begin{figure}[t]
% \vspace{-1mm}
	\centering
 
	\subfloat[\jdata]{\label{fig:baseline_rootcause_j}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/jdoctor_bl_rootcause.pdf}}
	
	
	\subfloat[\ddata]{\label{fig:baseline_rootcause_d}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/docter_bl_rootcause.pdf}}

 	\subfloat[\cdata]{\label{fig:baseline_rootcause_c}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/cmm_bl_rootcause.pdf}}
	   % \vspace{-1mm}

	\caption{Distributions of root causes for baselines' failures.}
	\label{fig:baseline_rootcause}
	% \vspace{-3mm}
   
\end{figure}




==> images/jdoctor_symptom_entity.tex <==
\begin{figure}[ht]
  \centering
  \subfloat[Jdoctor]{\label{fig:jdoctor_symptom}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.6\linewidth]{images/jdoctor_symptom.pdf}}
  \hfill
  \subfloat[Symptom]{\label{fig:docter_modelsize}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.4\linewidth]{images/num_entity.pdf}}
  \caption{Entity}
  \label{fig:entity}
\end{figure}

==> images/root_cause.tex <==

\begin{figure}[t]
% \vspace{-1mm}
	\centering
	\subfloat[\jdata]{\label{fig:jdoctor_rootcause}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/jdoctor_rootcause.pdf}}
	
	
	\subfloat[\ddata]{\label{fig:docter_rootcause}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/docter_rootcause.pdf}}

 	\subfloat[\cdata]{\label{fig:cmm_rootcause}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=\linewidth]{images/cmm_rootcause.pdf}}
	
    % \vspace{-1mm}
	\caption{Distributions of root causes of \basemodel's failures.}
	\label{fig:rootcause}
	% \vspace{-3mm}
   
\end{figure}



==> images/venn.tex <==
\begin{figure*}[t]
  \centering
  \subfloat[\jdata]{\label{fig:jdoctor_venn}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.27\linewidth]{images/Jdoctor_venn_v4.pdf}}
  % \hfill
  \subfloat[\ddata]{\label{fig:docter_venn}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.27\linewidth]{images/Docter_venn_v4.pdf}}
    \subfloat[\cdata]{\label{fig:cmm_venn}\includegraphics[clip=true,trim=0mm 0.5mm 0mm 0mm,width=0.27\linewidth]{images/CMM_venn_v4.pdf}}
  % \vspace{-1mm}
  \caption{Venn diagrams of specification generation. $L$: \basemodel;  $J$: \jdoctor; $D$: \docter; $C$: \callmemaybe.
  % \q{+} indicates correct, while \q{-} denotes incorrect results. 
  % The numbers are from the experiment using \basemodel with SR and $K=60$.
  }%\lin{People knows what Venn graph means. If you label Codex and Docter, it clear what the other cells mean. The color filling are unnecessary and bad.  See a  black white venn graph like Fig. 2 in  \url{https://www.cs.purdue.edu/homes/lintan/publications/opad-fse17.pdf}}\danning{updated}

  \label{fig:venn}
\end{figure*}



==> tables/rq3-callmemaybe-all.tex <==

\begin{table}[]
\caption{Comparison of different LLMs with SR on \cdata: Accuracy (\%), and Cost (\$).
}
\label{tab:rq3-cmm-all}
\small

\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular} {lccccc}

\toprule

\multicolumn{2}{c}{Approach / Model (+SR)} & K & Accuracy & Cost (\$) \\
\callmemaybe & & - & 70.0 & - \\
\midrule

\multirow{7}{*}{GPT} & \multirow{4}{*}{4} 
& 10 &  67.4 &2.5\\
&& 20 &  66.3 & 5.1\\
&& 40 &  65.2 & 10.1\\
&& 60 &  \textbf{70.8}  & 15.15\\
\cline{2-5}
 & \multirow{3}{*}{3.5} 
& 10 & \textbf{70.8} & 0.25 \\
&& 20 & \textbf{71.9 }& 0.51 \\
&& 40 & \textbf{73.0} & 1.01 \\

\midrule


\multirow{8}{*}{Codellama} & \multirow{4}{*}{13B} 
& 10 & \textbf{71.9}& - \\
&& 20 & \textbf{70.8}  & - \\
&& 40 & \textbf{75.3} & - \\
&&  60& \textbf{\benchmarkCMMSRSixty}& -\\
\cline{2-5}
 & \multirow{4}{*}{7B} 
& 10 & \textbf{73.0} & - \\
&& 20 & \textbf{75.3}& - \\
&& 40 & \textbf{74.2}& - \\
&& 60 & \textbf{75.3} & - \\


\midrule

\multirow{4}{*}{deepseek-coder} & \multirow{4}{*}{6.7B} 
& 10 & 67.4  & -\\
&& 20 & 66.3  & -\\
&& 40 &  66.3 & -\\
&& 60 &  66.3 & - \\
\midrule

\multirow{4}{*}{Llama3} & \multirow{4}{*}{8B} 
& 10 &  69.7 & -\\
&& 20 &  67.4& -\\
&& 40 &  \textbf{70.8} & -\\
&& 60 &  \textbf{71.9} & - \\
\midrule

\multirow{6}{*}{Llama2} & \multirow{3}{*}{13B} 
& 10 & 69.7& - \\
&& 20 & \textbf{74.2} & - \\
&& 40 & \textbf{73.0} & - \\

\cline{2-5}
& \multirow{3}{*}{7B} 

& 10 & 66.3& - \\
&& 20 & 68.5 & - \\
&& 40 & 69.7 & - \\
\midrule


\multirow{8}{*}{StarCoder2} & \multirow{4}{*}{15B} 
& 10 &  \textbf{75.3}  & -\\
&& 20 & \textbf{76.4}  & -\\
&& 40 & \textbf{76.4}  & -\\
&& 60 &  \textbf{75.3} & - \\
\cline{2-5}
& \multirow{4}{*}{7B} 
& 10 &  \textbf{74.2} & -\\
&& 20 &  \textbf{75.3} & -\\
&& 40 &  \textbf{76.4}  & -\\
&& 60 &  \textbf{76.4} & - \\


\midrule



\multirow{4}{*}{StarCoder} & \multirow{4}{*}{16B} 
& 10 & 62.9& - \\
&& 20 & 65.2  & - \\
&& 40 & \textbf{74.2} & - \\
&& 60 & \textbf{73.0} & - \\



\midrule




\multirow{4}{*}{CodeGen2} 
& \multirow{2}{*}{16B} 
& 10 & 67.4 & -  \\
&& 20 & 68.5 & -  \\
\cline{2-5}
 & \multirow{2}{*}{7B} 
& 10 & 68.5 & -  \\
&& 20 & 67.4 & -  \\

 \bottomrule

 
% \midrule
% \bottomrule
\end{tabular}
}
\end{table}

==> tables/rq3-docter-all.tex <==
\begin{table}[]
\caption{Comparison of different LLMs with SR on \ddata: Precision/Recall/F1 (\%), and Cost.  }
% \vspace{-1mm}
\label{tab:rq3-docter-all}
% \scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule

\multicolumn{2}{c}{Approach / Model (+SR)} & K & \multicolumn{1}{c}{TensorFlow} & \multicolumn{1}{c}{PyTorch} & \multicolumn{1}{c}{MXNet} & \multicolumn{1}{c}{Overall} & \multicolumn{1}{c}{Cost (\$)} \\
\midrule




 \docter &  & - & 90.0/74.8/81.7 & 78.4/77.4/77.9 &  87.9/82.4/85.1 & 85.4/78.2/\df & - \\

\midrule


\multirow{2}{*}{GPT} 
 & \multirow{4}{*}{4} 
 & 10 &  80.2/83.4/81.8 & 77.1/81.2/79.1 & 83.3/86.2/84.8 & 81.2/84.4/\textbf{82.8} & 13 \\
 && 20 &82.4/85.6/84.0 & 80.5/84.2/82.3 & 84.8/88.1/86.4 & 83.2/86.6/\textbf{84.9} &26 \\
 && 40 & 83.9/87.1/85.5 & 81.2/85.7/83.4 & 85.6/88.9/87.2 & 84.3/87.7/\textbf{86.0}& 52 \\
 && 60 & 84.7/87.5/86.1 & 82.8/87.3/85.0 & 86.8/89.9/88.3 & 85.4/88.6/\textbf{87.0}& 78 \\
  \cline{2-8}
 & \multirow{2}{*}{3.5} 
& 10 & 79.4/81.7/80.5 & 73.6/79.8/76.6 & 81.2/85.6/83.3 & 79.3/83.3/81.2 & 2.6 \\
 && 20 & 81.9/83.7/82.8 & 77.3/81.2/79.2 & 84.3/87.3/85.8 & 82.3/85.0/\textbf{83.6} & 5.2 \\


\midrule






\multirow{8}{*}{CodeLlama} & \multirow{4}{*}{13B} 
& 10 & 82.8/82.4/82.6 & 81.6/80.2/80.9 & 86.0/87.4/86.7 & 84.1/84.4/\textbf{84.3} & - \\
&& 20 & 84.1/84.4/84.2 & 83.6/82.7/83.1 & 86.6/88.4/87.5 & 85.2/86.0/\textbf{85.6} & - \\
&& 40 & 85.9/85.8/85.9 & 83.4/83.4/83.4 & 87.5/88.4/87.9 & 86.2/86.6/\textbf{86.4} & - \\
&& 60 & 85.0/86.7/85.8 & 83.4/84.6/84.0 & 87.4/89.2/88.3 & 85.9/87.5/\textbf{\codexDocTerSRFSixty} & - \\
 \cline{2-8}
& \multirow{4}{*}{7B} 
& 10 & 83.9/77.3/80.5 & 83.0/74.7/78.6 & 87.2/84.4/85.8 & 85.3/80.3/\textbf{82.7} & - \\
& & 20 & 86.5/81.1/83.7 & 83.3/76.0/79.5 & 87.5/86.6/87.0 & 86.4/82.9/\textbf{84.6} & - \\
& & 40 & 86.7/82.8/84.7 & 83.1/77.1/80.0 & 88.2/87.7/87.9 & 86.8/84.2/\textbf{85.4} & - \\
 && 60 & 86.4/83.6/85.0 & 84.4/80.4/82.4 & 88.2/88.8/88.5 & 86.9/85.6/\textbf{86.2} & - \\
\midrule







\multirow{4}{*}{deepseek-coder}
 & \multirow{4}{*}{6.7B}
  & 10 & 82.4/80.9/81.6 & 81.8/79.7/80.8 & 85.3/86.2/85.8 & 83.7/83.2/\textbf{83.5} & - \\
 && 20 &84.4/83.5/83.9 & 83.1/80.2/81.6 & 86.4/87.9/87.2 & 85.1/85.1/\textbf{85.1} & - \\
 && 40 & 85.5/85.4/85.5 & 83.7/81.9/82.8 & 87.4/88.1/87.8 & 86.1/86.1/\textbf{86.2} & - \\
 && 60 & 85.9/85.4/85.7 & 85.6/84.6/85.1 & 87.5/89.1/88.3 & 86.6/87.0/\textbf{86.9} & - \\
\midrule



\multirow{4}{*}{Llama3}
 & \multirow{4}{*}{8B}
  & 10 & 84.3/76.1/80.0 & 83.8/75.6/79.5 & 87.0/85.3/86.2 & 85.5/80.4/\textbf{82.9}  & - \\
 && 20 & 85.3/81.4/83.3 & 82.8/78.5/80.6 & 87.7/87.7/87.7 & 86.0/83.9/\textbf{85.0}   & - \\
 && 40 & 85.9/82.2/84.0 & 83.9/80.6/82.2 & 87.8/88.3/88.0 & 86.5/84.9/\textbf{85.6} & - \\
 && 60 & 86.1/82.8/84.4 & 83.3/83.0/83.1 & 87.7/85.6/86.7 & 86.4/84.2/\textbf{85.3}  & - \\
\midrule
\multirow{4}{*}{Llama2}
 & \multirow{2}{*}{13B}
& 10 & 82.3/76.4/79.3 & 81.1/73.4/77.1 & 85.9/82.4/84.1 & 83.8/78.8/81.2 & - \\
&& 20 & 83.9/80.0/81.9 & 80.4/74.2/77.2 & 84.4/81.3/82.8 & 83.6/79.6/81.5 & - \\

\cline{2-8}


& \multirow{2}{*}{7B}
& 10 & 78.2/77.7/78.0 & 75.2/73.5/74.3 & 82.6/83.2/82.9 & 79.8/79.6/79.7 & - \\
&& 20 &  80.5/79.2/79.8 & 77.7/75.5/76.6 & 84.0/80.6/82.3 & 81.7/79.3/80.5 & - \\
\midrule




% \midrule
\multirow{8}{*}{StarCoder2} & \multirow{4}{*}{15B} 
  & 10 & 85.4/82.4/83.9 & 83.4/79.6/81.4 & 86.6/86.4/86.5 & 85.6/83.9/\textbf{84.7} & - \\
 && 20 &  86.6/85.4/86.0 & 84.2/81.8/83.0 & 87.5/88.4/88.0 & 86.6/86.2/\textbf{86.5} & - \\
 && 40 & 87.4/86.7/87.1 & 84.6/84.1/84.3 & 87.6/88.7/88.2 & 87.0/87.2/\textbf{87.2} & - \\
&& 60&  87.9/87.2/87.6 & 85.8/85.4/85.6 & 88.6/89.4/89.0 & 87.9/88.0/\textbf{87.9}& - \\
\cline{2-8}
& \multirow{4}{*}{7B} 
  & 10 & 83.6/81.0/82.3 & 82.7/79.4/81.0 & 86.6/86.6/86.6 & 84.9/83.4/\textbf{84.2}  & - \\
 && 20 & 85.5/84.1/84.8 & 83.2/82.6/82.9 & 87.1/88.4/87.7 & 85.9/85.9/\textbf{85.9}  & - \\
 && 40 & 86.2/85.8/86.0 & 83.7/84.1/83.9 & 87.4/89.0/88.2 & 86.4/87.1/\textbf{86.7}  & - \\
&& 60 & 86.8/86.7/86.7 & 84.8/85.4/85.1 & 87.7/89.1/88.4 & 86.9/87.6/\textbf{87.2}  & - \\
\midrule

\multirow{4}{*}{StarCoder} & \multirow{4}{*}{16B} 
& 10 & 81.9/81.7/81.8 & 79.7/77.1/78.4 & 86.3/86.1/86.2 & 83.6/83.0/\textbf{83.3} & -  \\
&& 20 & 83.2/84.4/83.8 & 81.3/80.7/81.0 & 86.8/88.1/87.5 & 84.6/85.6/\textbf{85.1} & -  \\
&& 40 & 84.8/86.1/85.4 & 82.6/83.1/82.8 & 87.6/89.0/88.3 & 85.8/87.0/\textbf{86.4} & -  \\
&& 60 & 85.0/86.7/85.8 & 83.4/84.6/84.0 & 87.4/89.2/88.3 & 85.9/87.5/\textbf{86.7} & -  \\

\midrule





\multirow{2}{*}{CodeGen2}
& \multirow{1}{*}{16B} 
& 10 & 79.7/81.4/80.6 & 77.6/79.3/78.5 & 85.0/86.3/85.7 & 81.9/83.4\textbf{/82.7} & - \\
\cline{2-8}
& \multirow{1}{*}{7B} 
& 10 & 77.7/77.3/77.5 & 76.6/77.2/76.9 & 82.2/84.0/83.1 & 79.7/80.5/80.1 & - \\



\bottomrule
\end{tabular}%
}
\end{table}





==> tables/rq3-jdoctor-all.tex <==
\begin{table}[]
\caption{Comparison of different LLMs with SR on \jdata: Accuracy (\%) and Cost.}
\label{tab:rq3-jdoctor-all}
% \vspace{-1mm}
% \scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Approach/\\ Model (+SR)\end{tabular}}}  & \multirow{2}{*}{K} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% Precond\\ 
\texttt{@param}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% Normal\\ postcond\\ 
\texttt{@return}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}
% Exceptional\\ postcond\\ 
\texttt{@throws}\end{tabular}} &\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Overall\end{tabular}} & 
{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cost\\ (\$)\end{tabular}}}
\\ \cline{4-11} 

 & & & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Processed} & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Processed} & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Processed} & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Processed} \\


 
 \midrule
\jdoctor & & - & 97.0 & 97.0 & 69.0 & 69.0 & 79.0 & 79.0 & \jacc & \jacc  & - \\
\midrule

\multirow{8}{*}{GPT} 
& \multirow{4}{*}{4} 
& 10 & 88.1 & 95.9   & 53.2 & 72.7&  84.1 & 91.5&  80.2 &\textbf{89.7}   &  19.5  \\
&& 20 & 89.7 & 95.9 &  60.4& 77.7&  86.2 &92.8 & 83.0  &\textbf{91.2}   &  39.0  \\
&& 40 &  89.3& 95.9 & 58.3 & 75.5& 88.8  &94.5 & 84.0  &\textbf{91.8}   &   78 \\
&& 60 &  90.1 & 95.5 &  63.3 & 77.7  &90.0   & 94.9  &  85.7 & \textbf{92.3} & 117 \\
\cline{2-12}
& \multirow{4}{*}{3.5} 
& 10 & 86.9 & 93.5 & 60.8 & 70.9 & 81.6 & 91.0 & 80.6 & \textbf{89.3} & 1.3  \\
&& 20 & 82.0 & 89.1 & 60.8 & 72.2 & 83.5 & 90.3 & 80.4 & \textbf{87.9} & 2.6  \\
&& 40 & 83.6 & 89.6 & 59.5 & 74.7 & 84.5 & 88.8 & 81.3 & \textbf{87.4} & 5.2  \\
&& 60 & 86.3 & 89.1 & 59.5 & 72.2 & 80.1 & 84.7 & 79.4 & \textbf{84.4} & 7.8  \\
\midrule




\multirow{8}{*}{Codellama} & \multirow{4}{*}{13B} 
& 10 & 93.0 & 96.7 & 62.6 & 71.2 & 84.5 & 90.3 & 83.4 & \textbf{89.0}  & -  \\
& & 20 & 94.7 & \textbf{97.5} & 63.3 & 73.4 & 86.4 & 91.3 & 85.0 & \textbf{90.2}  & -  \\
&& 40 & 95.9 & 97.9 & 62.6 & 72.7 & 89.6 & 94.7 & 87.0 & \textbf{82.0}  & -  \\
&& 60 & 95.9 & 98.8 & 65.5 & 75.5 & 90.3 & 96.0 & 87.9& \textbf{93.5}  & -  \\
\cline{2-12}
& \multirow{4}{*}{7B} 
& 10 & 92.2 & 96.3 & 60.4 & 71.2 & 84.5 & 90.5 & 82.8 & \textbf{89.0} & -  \\
&& 20 & 93.8 & 97.9 & 64.0 & 74.8 & 86.2 & 91.9 & 84.7 & \textbf{90.8} & -  \\
&& 40 & 93.8 & 97.5 & 61.9 & 75.5 & 89.2 & 92.6 & 86.1 & \textbf{91.2} & -  \\
&& 60 & 95.5 & 98.4 & 60.4 & 72.7 & 90.9 & 95.3 & 87.2 & \textbf{92.5} & -  \\
\midrule





% \midrule
\multirow{4}{*}{deepseek-coder}
 & \multirow{4}{*}{6.7B}
& 10 & 90.9 & 95.9 & 61.9 & 74.1& 84.3  & 91.1 & 82.5  &  \textbf{89.7} &  -  \\
&& 20 & 93.8 &  97.5& 64.0&67.5 &  86.4 & 92.6&  84.9 &  \textbf{90.0} &  -  \\
&& 40 & 93.4 & 96.7 & 60.4 & 65.5 &  90.5 & 94.9&  86.4 &  \textbf{90.6}& -   \\
&& 60 &  93.8 & 96.3 &  60.4 & 71.2  & 91.5  & 96.0  & 87.1  &\textbf{92.0}  & - \\


\midrule

\multirow{4}{*}{Llama3}
 & \multirow{4}{*}{8B}
& 10 & 90.5 &  95.5& 63.3 & 66.9& 83.3  & 90.3& 82.1  &   \textbf{88.0}&   -\\
&& 20 & 93.8 & 97.5 &66.2  & 69.8&  86.7 & 92.6 &  85.4 &  \textbf{90.3}  & -   \\
&& 40 &  95.1&  97.1 & 60.4 & 63.3 & 89.0  & 94.1& 86.1  &  \textbf{89.9} &  -  \\
&& 60 &  95.9 & 96.4 &  65.5 & 77.7  & 90.0  & 94.5  & 87.1  &\textbf{92.9}  & - \\
% \cline{2-12}
\midrule 
\multirow{8}{*}{Llama2}
 & \multirow{4}{*}{13B}
& 10 & 91.4 & 96.3 & 58.3 & 66.9 & 81.6 & 85.8 & 80.6 &\textbf{85.7} & - \\
&& 20 & 93.0 & 96.7 & 60.4 & 66.9 & 83.5 & 87.9 & 82.4 & \textbf{87.0} & - \\
&& 40 & 94.2 & 96.7 & 59.0 & 65.5 & 86.9 & 91.9 & 84.4 & \textbf{89.0} & - \\
&& 60 & 95.1 & 98.4 & 56.8 & 68.3 & 88.6 & 93.0 & 85.3 & \textbf{90.5} & - \\
\cline{2-12}
& \multirow{4}{*}{7B}
& 10 & 88.9 & 93.0 & 56.8 & 64.7 & 77.5 & 82.0 & 77.4 & 82.3 & - \\
&& 20 & 91.4 & 95.9 & 56.1 & 66.9 & 82.8 & 86.7 & 80.9 &\textbf{86.1} & - \\
&& 40 & 94.2 & 95.9 & 58.3 & 67.6 & 86.2 & 91.7 & 83.9 & \textbf{89.0} & - \\
&& 60 & 95.1 & 97.5 & 56.1 & 67.6 & 86.9 & 91.7 & 84.2 & \textbf{89.4} & - \\
% \midrule


\midrule
\multirow{8}{*}{StarCoder2} & \multirow{4}{*}{15B} 
& 10 & 91.8 & 97.1 &61.9  & 71.9 & 83.1  &89.8 & 82.1  & \textbf{89.0}  &   - \\
&& 20 &94.7  & 97.5  &64.0  & 73.4& 87.1  & 92.6 &  85.5 &   \textbf{90.9}& -   \\
&& 40 & 95.1 & 97.5 &64.0  & 78.4& 89.4  &94.3 &86.9   & \textbf{92.6}   & -   \\
&& 60 & 96.3  & 98.4 98.4& 65.0  &77.7& 91.7  &95.6   & 88.7  & \textbf{93.5} & - \\
\cline{2-12}
& \multirow{4}{*}{7B} 
& 10 &  92.2& 93.2 & 59.0 & 67.6&  83.7 & 90.3 &  82.1 &  \textbf{87.4} &-    \\
&& 20 & 93.8 & 93.2 & 63.3 & 71.9&  85.8 & 91.7&  84.4 &  \textbf{88.9}  &-    \\
&& 40 & 95.1  & 97.0  & 61.2 & 74.8&  88.8 & 93.2 & 86.1  & \textbf{91.3}  &  -  \\
&& 60 &  95.9 & 97.9 &  64.0 & 76.3  &90.5   & 94.5  & 87.7  &\textbf{92.5}  & - \\

\midrule
\multirow{4}{*}{StarCoder} & \multirow{4}{*}{16B} 
& 10 & 91.8 & 95.4 & 63.3 & 74.1 & 83.9 & 90.0 & 82.8 & \textbf{88.9} & - \\
&& 20 & 94.2 & 97.9 & 65.5 & 78.4 & 86.2 & 91.1 & 85.1 & \textbf{91.0} & - \\
&& 40 & 95.1 & 97.9 & 63.3 & 74.8 & 88.8 & 93.4 & 86.4 & \textbf{91.7} & - \\
&& 60 & 95.9 & 98.4 & 64.7 & 77.7 & 90.3 & 94.7 & 87.7 & \textbf{93.0} & - \\

\midrule




\multirow{4}{*}{CodeGen2}
& \multirow{2}{*}{16B} 
& 10 & 93.4 & 97.8 & 59.5 & 68.4 & 81.6 & 85.0 & 82.2 & \textbf{86.5} & -  \\
&& 20 & 93.4 & 98.9 & 60.8 & 70.9 & 84.2 & 88.1 & 84.0 & \textbf{89.0} &- \\
\cline{2-12}
 & \multirow{2}{*}{7B} 
 & 10 & 89.6 & 95.1 & 64.6 & 70.9 & 77.9 & 80.8 & 79.5 & \textbf{83.5} & -  \\
&& 20 & 91.8 & 96.7 & 64.6 & 72.2 & 84.5 & 87.6 & 84.2 & \textbf{88.3} & -  \\


\bottomrule
\end{tabular}%
}
\end{table}



